MULTI-FLGANs: Multi-Distributed Adversarial Networks for Non-IID distribution

Federated learning is an emerging concept in the domain of distributed machine learning. This concept has enabled GANs to benefit from the rich distributed training data while preserving privacy. However, in a non-iid setting, current federated GAN architectures are unstable, struggling to learn the distinct features and vulnerable to mode collapse. In this paper, we propose a novel architecture MULTI-FLGAN to solve the problem of low-quality images, mode collapse and instability for non-iid datasets. Our results show that MULTI-FLGAN is four times as stable and performant (i.e. high inception score) on average over 20 clients compared to baseline FLGAN.

==> sections/abstract.tex <==
\begin{abstract}
Federated learning is an emerging concept in the domain of distributed machine learning. This concept has enabled GANs to benefit from the rich distributed training data while preserving privacy.  However, in a non-iid setting, current federated GAN architectures are  unstable, struggling to learn the distinct features and  vulnerable to mode collapse. In this paper, we propose a novel architecture MULTI-FLGAN to solve the problem of low-quality images, mode collapse and instability for non-iid datasets. Our results show that MULTI-FLGAN is four times as stable and performant (i.e. high inception score) on average over 20 clients compared to baseline FLGAN.


% A recent technical breakthrough in the domain of
% machine learning is the discovery and the multiple applications
% of Generative Adversarial Networks (GANs). Those generative
% models are computationally demanding, as a GAN is composed
% of two deep neural networks, and because it trains on large
% datasets. A GAN is generally trained on a single server.
% In this paper, we address the problem of distributing GANs
% so that they are able to train over datasets that are spread on
% multiple workers. MD-GAN is exposed as the first solution for
% this problem: we propose a novel learning procedure for GANs
% so that they fit this distributed setup. We then compare the
% performance of MD-GAN to an adapted version of federated
% learning to GANs, using the MNIST, CIFAR10 and CelebA
% datasets. MD-GAN exhibits a reduction by a factor of two of
% the learning complexity on each worker node, while providing
% better or identical performances with the adaptation of federated learning. 
\end{abstract}

==> sections/conclusion_and_future_work.tex <==
\section{Conclusions and Future Work}


==> sections/responsible_research.tex <==
\section{Responsible Research}
Reflect on the ethical aspects of your research and discuss the reproducibility of your methods.
Note that although in many published works there is no such a section (it may be part of some meta-information collected by the journal, or part of the discussion section), we require you to think (and report) about this as part of this course.

==> sections/your_contribution.tex <==
\section{Your contribution (replace this section title by something more informative)}
In computer science typically the third section contains an exposition of the main ideas, for example the development of a theory, the analysis of the problem (some proofs), a new algorithm, and potentially some theoretical analysis of the properties of the algorithm.

Do not forget to give this section another name, for example after the method or idea you are presenting.

Some more detailed suggestions for typical types of contributions in computer science are described in the following subsections.


\subsection*{Experimental work}
In this case, this section will mostly contain a description of the methods/algorithms you will be comparing. Although not all methods need to be described in detail (providing appropriate references are available), make sure that you reveal sufficient details to a reader not familiar with these methods to: a) obtain a high-level understanding of the method and differences between them, and b) understand your explanation of the results/conclusions.

\subsection*{Improvement of an idea}
In this case, you would need to explain in detail how the improvement works. If it is based on some observation that can be proven, this is a good place to provide that proof (e.g., of the correctness of your approach). 

\subsection*{Literature survey}
If your contribution is a literature survey, then the organization of these ``middle'' sections very much depends on the way you want to present/organize the literature you are discussing.
First try to cluster papers that are similar in some aspect. Then think of how these clusters are related, from that you can think of a good order to discuss these clusters; this is sometimes called a bottom-up approach to writing a paper.

In addition, you may try to think about the organization of the literature from a top-down perspective: try to ``take a step back'' and think about the field and what important questions/variants are and build a hierarchical categorization of the field.

Make clear what your contribution is here: a new organization of the literature, identification of open problems/challenges, new parallels/generalizations, a table with pros/cons of different methods, etc.\ 


